INGRID: an interactive grid generator for 2D edge plasma modeling

A fusion boundary-plasma domain is defined by axisymmetric magnetic surfaces where the geometry is often complicated by the presence of one or more X-points; and modeling boundary plasmas usually relies on computational grids that account for the magnetic field geometry. The new grid generator INGRID (Interactive Grid Generator) presented here is a Python-based code for calculating grids for fusion boundary plasma modeling, for a variety of configurations with one or two X-points in the domain. Based on a given geometry of the magnetic field, INGRID first calculates a skeleton grid which consists of a small number of quadrilateral patches; then it puts a subgrid on each of the patches, and joins them in a global grid. This domain partitioning strategy makes possible a uniform treatment of various configurations with one or two X-points in the domain. This includes single-null, double-null, and other configurations with two X-points in the domain. The INGRID design allows generating grids either interactively, via a parameter-file driven GUI, or using a non-interactive script-controlled workflow. Results of testing demonstrate that INGRID is a flexible, robust, and user-friendly grid-generation tool for fusion boundary-plasma modeling.

==> classification/index_space_layout.tex <==
\subsection{Index space layout}

==> classification/one_x_point_case.tex <==
\subsection{One x-point}
In the case of the primary x-point, we define N to be in the direction
of decreasing $\Psi$ towards the magnetic-axis, and S to be in the
direction of decreasing $\Psi$ towards the private-flux region. We
assign a Point object for the N and S $(r,z)$ coordinates some small
$\epsilon$ distance away from the primary x-point in order to provide
the LineTracing class a starting point towards the magnetic-axis and
private-flux region. To define E, W, NE, NW, SE, and SE, we simply
apply the appropriate rotations to the established N and S directions
of the primary x-point. The above results in a group of Point objects
located a distance $\epsilon$ away from the primary x-point.\\ \indent
To highlight the significance of this convention, consider an SNL
divertor configuration. Using the primary x-point N-S-E-W definitions
used above, it can be seen that the to trace the primary separatrix,
we simply perform LineTracing from the SW, SE, NW, and NE
directions. This holds for both LSN and USN cases. Going further, we
no longer rely on a notion of ``inner" and ``outer" for target plates,
and can now utilize a general N-S-E-W direction to specify which
target plate we are speaking of. In a typical LSN case, the ``inner"
target plate is equivalently ``SW" of the primary x-point. Similarly,
the ``outer" target plate is equivalently ``SE" of the primary
x-point. We refer to these plates in the INGRID parameter file and
documentation as ``plate\_W1" and ``plate\_E1". The W and E correspond
to the ``SW" and ``SE" directions, whereas the ``1" indicates these
plates correspond to the primary x-point dubbed ``xpt1".


==> classification/two_x_point_case.tex <==
\subsection{Two x-points}
For understanding the N-S-E-W convention of the secondary x-point, it is useful to consider the partition of the domain induced by any given separatrix. With these distinct regions in mind, we define N for the secondary x-point to be the in the direction of the region that contains the primary separatrix. We assign a Point object for this N direction some $\varepsilon$ distance away from the secondary x-point. The remaining secondary x-point directions (S, E, W, SE, SW, NE, NW) are obtained by the appropriate rotations of the established N Point.\\ \indent
This secondary x-point N-S-E-W criteria is not only a critical step for identification of a divertor configuration, but also provides a general plate naming scheme for all magnetic topologies. Just like the primary x-point case, we have the ``SW" and ``SE" directions of the secondary x-point intersect individual target plates. We can see this idea and the ideas discussed earlier in figure \ref{fig:xpt_2_directions}. To remain consistent with the primary x-point target plate naming scheme, we refer to these plates as ``plate\_W2" and ``plate\_E2" for the ``SW" and ``SE" directions respectively. The ``2" here indicates that these plates are unique to the cases with two x-points.


==> classification/x_point_notation.tex <==
\subsection{N-S-E-W notation}
In this section we detail INGRID's approach to analysis of x-points. The user begins by specifying the number of x-points INGRID should take into consideration. INGRID takes this information to determine which identification scheme to utilize. In all cases, however, INGRID defines a notion of ``North" (N), ``South" (S), ``East" (E), and ``West" (W) directions for each x-point. By defining these N-S-E-W directions, INGRID can identify the divertor configuration within the EFIT data. We utilize a specific method of assigning N-S-E-W directions depending on which x-point we are analyzing (i.e. primary x-point or secondary x-point).

==> computation/handling_target_plates.tex <==
\subsection{Handling of target plates}
INGRID users must specify the geometry of the limiter (by which we
mean here the entire first-wall contour surrounding the plasma)
and/or target
plates, to represent the shape of material walls in a modeled
device. The limiter and target plates are represented in INGRID by a
piecewise-linear model defined by a set of nodes; the (R,Z)
coordinates of those nodes are expected to be provided in separate
data files. There is one data file for the limiter and one for each
target plate, either in the text format or as a NumPy binary. The
names of those data files are set in the INGRID parameter file. In the
case that the limiter and target plate data are provided in text
format, the user must specify (r,z) coordinates for each point
defining the surface sequentially on a separate line in the
corresponding data file; and Python-formatted single- line comments
can be included, as shown in the Appendix.  For use of NumPy binary
files, users must also adhere to a particular internal file
structure. Given two NumPy arrays of shape $(n,:)$ that represent $R$
and $R$ coordinate values respectively, one can define a NumPy array
of shape $(2,n)$ representing the $n$-many points required to model
the piecewise-linear model of interest. This NumPy array of shape $(2,
n)$ can be saved into a NumPy binary file in order to be loaded into
INGRID.  In addition to the requirements above, INGRID asserts that
strike-point geometry files used for Patch maps are monotonic in $\Psi$
along the length of the target plates (i.e. no shadow regions). This
assertion allows for INGRID generated Patch maps to conform entirely
to a user's specified strike-point geometry. While operating INGRID in
GUI mode, the user will be warned if the loaded geometry file is not
monotonic in $\Psi$ along the target plate length.

